Dataset Condensation with Differentiable Siamese Augmentation

In many machine learning problems, large-scale datasets have become the de-facto standard to train state-of-the-art deep networks at the price of heavy computation load. In this paper, we focus on condensing large training sets into significantly smaller synthetic sets which can be used to train deep neural networks from scratch with minimum drop in performance. Inspired from the recent training set synthesis methods, we propose Differentiable Siamese Augmentation that enables effective use of data augmentation to synthesize more informative synthetic images and thus achieves better performance when training networks with augmentations. Experiments on multiple image classification benchmarks demonstrate that the proposed method obtains substantial gains over the state-of-the-art, 7% improvements on CIFAR10 and CIFAR100 datasets. We show with only less than 1% data that our method achieves 99.6%, 94.9%, 88.5%, 71.5% relative performance on MNIST, FashionMNIST, SVHN, CIFAR10 respectively. We also explore the use of our method in continual learning and neural architecture search, and show promising results.

==> table_abstudy_fromnoise.tex <==
\begin{table*}[]
\centering
\scriptsize
\begin{tabular}{ccccccccccc}
\toprule
     & \multicolumn{2}{c}{Condense}    & Test      & \multicolumn{7}{c}{Test Performance (\%)} \\ 
     & Real           & Synthetic      & Synthetic & Color          & Crop          & Cutout        & Flip          & Scale         & Rotation  & Combination \\ \midrule
Ours & $\ma_{\omega}$ & $\ma_{\omega}$ & $\ma$     & 47.4$\pm$0.5  & 48.9$\pm$0.6  & 47.8$\pm$0.6  & 47.5$\pm$0.6  & 47.0$\pm$0.5  & 46.8$\pm$0.5  & 51.4$\pm$0.5\\ \midrule
(A)  & -              & -              & -         & 44.9$\pm$0.5  & 44.9$\pm$0.5  & 44.9$\pm$0.5  & 44.9$\pm$0.5  & 44.9$\pm$0.5  & 44.9$\pm$0.5  & 44.9$\pm$0.5\\
(B)  & -              & -              & $\ma$     & 46.6$\pm$0.6  & 46.8$\pm$0.6  & 47.6$\pm$0.6  & 45.8$\pm$0.7  & 44.7$\pm$0.6  & 43.9$\pm$0.6  & 50.4$\pm$0.4\\
(C)  & $\ma$          & -              & $\ma$     & 46.4$\pm$0.5  & 43.6$\pm$0.7  & 46.2$\pm$0.6  & 46.0$\pm$0.7  & 44.3$\pm$0.6  & 44.0$\pm$0.6  & 49.6$\pm$0.4\\
(D)  & -              & $\ma$          & $\ma$     & 45.8$\pm$0.5  & 45.5$\pm$0.6  & 44.5$\pm$0.6  & 46.5$\pm$0.5  & 45.4$\pm$0.6  & 46.2$\pm$0.6  & 48.0$\pm$0.5\\
(E)  & $\ma_{\omega}$ & $\ma_{\omega}$ & -         & 45.1$\pm$0.5  & 43.6$\pm$0.5  & 42.3$\pm$0.7  & 46.3$\pm$0.5  & 45.4$\pm$0.5  & 46.1$\pm$0.6  & 44.5$\pm$0.6\\
(F)  & $\ma$          & $\ma$          & $\ma$     & 45.8$\pm$0.6  & 44.7$\pm$0.6  & 44.6$\pm$0.5  & 46.5$\pm$0.6  & 45.0$\pm$0.7  & 45.9$\pm$0.7  & 46.7$\pm$0.6\\
\bottomrule
\end{tabular}
\caption{\footnotesize{Ablation study on augmentation schemes in CIFAR10 for 10 synthetic image/class. $\ma_{\omega}$ denotes Siamese augmentation when applied to both real and synthetic data, while $\ma$ denotes augmentation that is not shared across different minibatches. Initialized from random noise.}}
\label{tab:abstudy_effectiveness_noise}
\vspace{-12pt}
\end{table*}

==> table_sota_Generator.tex <==
\begin{table}
% \vspace{-10pt}
\renewcommand\arraystretch{0.9}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{cccccc}
\toprule
        & Img/Cls & Ratio \% & DC           & GDC           & GDC+DSA      \\ \midrule
MNIST   & 1       & 0.017    & 91.7$\pm$0.5 & 85.4$\pm$0.7  & 88.4$\pm$0.6 \\
        & 10      & 0.17     & 97.4$\pm$0.2 & 95.9$\pm$0.2  & 97.6$\pm$0.1             \\ \midrule
F.MNIST & 1       & 0.017    & 70.5$\pm$0.6 & 69.8$\pm$0.8  & 69.7$\pm$0.8 \\
        & 10      & 0.17     & 82.3$\pm$0.4 & 81.2$\pm$0.3  & 82.9$\pm$0.3 \\ \midrule
SVHN    & 1       & 0.014    & 31.2$\pm$1.4 & 31.1$\pm$1.6  & 31.2$\pm$2.2 \\
        & 10      & 0.14     & 76.1$\pm$0.6 & 75.3$\pm$0.7  & 77.5$\pm$0.6 \\ \midrule
CIFAR10 & 1       & 0.02     & 28.3$\pm$0.5 & 28.0$\pm$0.8  & 28.7$\pm$0.9 \\
        & 10      & 0.2      & 44.9$\pm$0.5 & 43.1$\pm$0.5  & 49.3$\pm$0.5 \\
\bottomrule
\end{tabular}
\caption{\footnotesize{The performance comparison on generator based models.}}
\label{tab:sota_generator}
% \vspace{-5pt}
\end{table}

